Maximizing Uncertainty for Federated learning via Bayesian Optimisation-based Model Poisoning

As we transition from Narrow Artificial Intelligence towards Artificial Super Intelligence, users are increasingly concerned about their privacy and the trustworthiness of machine learning (ML) technology. A common denominator for the metrics of trustworthiness is the quantification of uncertainty inherent in DL algorithms, and specifically in the model parameters, input data, and model predictions. One of the common approaches to address privacy-related issues in DL is to adopt distributed learning such as federated learning (FL), where private raw data is not shared among users. Despite the privacy-preserving mechanisms in FL, it still faces challenges in trustworthiness. Specifically, the malicious users, during training, can systematically create malicious model parameters to compromise the models predictive and generative capabilities, resulting in high uncertainty about their reliability. To demonstrate malicious behaviour, we propose a novel model poisoning attack method named Delphi which aims to maximise the uncertainty of the global model output. We achieve this by taking advantage of the relationship between the uncertainty and the model parameters of the first hidden layer of the local model. Delphi employs two types of optimisation , Bayesian Optimisation and Least Squares Trust Region, to search for the optimal poisoned model parameters, named as Delphi-BO and Delphi-LSTR. We quantify the uncertainty using the KL Divergence to minimise the distance of the predictive probability distribution towards an uncertain distribution of model output. Furthermore, we establish a mathematical proof for the attack effectiveness demonstrated in FL. Numerical results demonstrate that Delphi-BO induces a higher amount of uncertainty than Delphi-LSTR highlighting vulnerability of FL systems to model poisoning attacks.

==> biography.tex <==
\begin{document}
\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Biography/marios_aristodemou_ieee.JPEG}
]
{Marios Aristodemou}
received the MEng Systems Engineering degree from Loughborough University, U.K in 2021. 
He has finished his Ph.D. degree with the Wolfson School of Mechanical, Electrical and Manufacturing Engineering, Loughborough University, U.K. He is currently a Post Doctoral Research Associate in University of York. He has being involved in various projects in Wireless Communications and Cyber Security, applying distributed learning and reinformcenet learning.
His research interests include the Artificial Intelligence and Metaverse, including topics such as the security and trustworthiness, personalised distributed learning, privacy preserving for distributed learning and lifelong learning. 

\includegraphics[width=1.2in,height=1.25in,clip,keepaspectratio]{Biography/xiaolan.jpeg}
{Xiaolan Liu }
received the Ph.D. degree from Queen Mary University of London, U.K. in 2021. She was a Research Associate at King’s College London from 2020-2021. She was a Lecturer at Loughborough
University London from 2021-2024. Since 2024, she has been a Lecturer with School of Electrical, Electronic and Mechanical Engineering at University of Bristol, U.K. Her current research interests include wireless distributed learning, multi-agent reinforcement learning for edge computing, and machine learning for wireless communication optimization. 

\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Biography/wangyuan_avatar.jpg}

{Yuan Wang}
received his Ph.D. degree from Nanyang Technological University, Singapore. He is now a senior scientist with the department of Computing and Intelligence, Institute of High Performance Computing, under A*STAR, Singapore. His current research mainly focus on decentralized and trustworthy AI, with a spotlight on Federated Learning, data synthesis techniques like dataset distillation and generative methods, large foundation models and related MedTech applications. 

\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Biography/kostas.jpg}
{Konstantinos G. Kyriakopoulos}~(IEEE Senior Member, IET member)~received the BSc degree in electrical engineering from the Technological Education Institute of Larisa, Greece, in 2003, the MSc degree in digital communication systems, and the PhD degree in computer networks from Loughborough University, Loughborough, UK, in 2004 and 2008, respectively. From 2008 to 2015, he was a Research Associate with the School of Electronic, Electrical, and Systems Engineering, Loughborough University, conducting research in mainly EPSRC projects and successfully licensing research output from his work. Since 2016, he has been an academic member with the Wolfson School of Mechanical, Electronic and Manufacturing Engineering at Loughborough University. His research interests are in the areas of intelligent decision making using machine learning, Evidence Theory, and soft computing techniques. He has extensive experience in computer network security, anomaly detection, contextual awareness, and performance measurements in emerging network paradigms and their applications.

\includegraphics[width=1in,height=1.25in,clip,keepaspectratio{Biography/Sangarapillai_lambotharan.jpg}
{Sangarapillai Lambotharan} received the Ph.D. degree in signal processing from Imperial College London, U.K., in 1997. He was a Visiting Scientist with the Engineering and Theory Centre, Cornell University, USA, in 1996. Until 1999, he was a Post-Doctoral Research Associate with Imperial College London. From 1999 to 2002, he was with the Motorola Applied Research Group, U.K., where he investigated various projects, including physical link layer modeling and performance characterization of GPRS, EGPRS, and UTRAN. He was with King’s College London and Cardiff University as a Lecturer and a Senior Lecturer, respectively, from 2002 to 2007. He is currently a Professor of Signal Processing and Communications and the Director of the Institute for Digital Technologies, Loughborough University London, U.K. His current research interests include 5G networks, MIMO, blockchain, machine learning, and network security. He has authored more than 250 journal articles and conference papers in these areas. He is a Fellow of IET and Senior Member of IEEE. He serves as a Senior Area Editor for the IEEE Transactions on Signal Processing and as an Associate Editor IEEE Transactions on Communications

\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Biography/qingsong_wei.jpg}
{Qingsong Wei} received the PhD degree in computer science from the University of Electronic Science and Technologies of China, in 2004. He was with Tongji University as an assistant professor from 2004 to 2005. He is a Group Manager and Principal Scientist at the Institute of High Performance Computing, A*STAR, Singapore. His research interests include decentralized computing, federated learning, privacy-preserving AI and Blockchain. He is a senior member of the IEEE
\end{document}

